Pollux: Co-adaptive Cluster Scheduling for Goodput-Optimized Deep Learning

Pollux improves scheduling performance in deep learning (DL) clusters by adaptively co-optimizing inter-dependent factors both at the per-job level and at the cluster-wide level. Most existing schedulers expect users to specify the number of resources for each job, often leading to inefficient resource use. Some recent schedulers choose job resources for users, but do so without awareness of how DL training can be re-optimized to better utilize the provided resources. Pollux simultaneously considers both aspects. By monitoring the status of each job during training, Pollux models how their goodput (a novel metric we introduce that combines system throughput with statistical efficiency) would change by adding or removing resources. Leveraging these information, Pollux dynamically (re-)assigns resources to improve cluster-wide goodput, while respecting fairness and continually optimizing each DL job to better utilize those resources. In experiments with real DL jobs and with trace-driven simulations, Pollux reduces average job completion times by 37-50% relative to state-of-the-art DL schedulers, even when they are provided with ideal resource and training configurations for every job. Pollux promotes fairness among DL jobs competing for resources based on a more meaningful measure of useful job progress, and reveals a new opportunity for reducing DL cost in cloud environments. Pollux is implemented and publicly available as part of an open-source project at https://github.com/petuum/adaptdl.

==> discussion.tex <==
\section{Discussion and Future Work}

\oursystem{} lies at the intersection between systems-oriented work on cluster resource scheduling and algorithms-oriented work on distributed DL training. We showed that 

\aurick{Can drop this.}

==> reviews.tex <==
\onecolumn
\begin{lstlisting}
OSDI '20 Paper #228 Reviews and Comments
===========================================================================
Paper #228 Pollux: Co-adaptive Cluster Scheduling for Goodput-Optimized
Deep Learning


Review #228A
===========================================================================

Paper summary
-------------
The paper defines the notion of goodput for deep learning (DL) training to take into account statistical efficiency, in addition to throughput. Pollux is a new cluster scheduling scheme for deep learning (DL) guided by goodput. Pollux manages to improve scheduling performance significantly by observing and adapting to the change of statistical efficiency in DL training. The adaptation happens both at the per-job level and the cluster-wide level, and has been shown to be effective compared to state-of-the-art DL schedulers.

Strengths
---------
 Definition of goodput. For deep learning training, taking into account statistical efficiency does lead to a better metric to guide the optimization. 

 Pollux mechanism of adaptations in response to changes in statistical efficiency opens up interesting opportunities for optimizations, both locally and globally. It is shown to outperform state-of-the-art schedulers.

Significant Weaknesses
----------------------
- There is a general lack of system perspectives and system-level innovations in the design of Pollux. The approach is mostly model and learning based. Pollux relies heavily on a prediction model for statistical efficiency; the model focuses only on DL metrics like batch size and learning rate, but does not go to the system-level decisions around the number of GPUs or distributed training. 

- The use of genetic algorithm for global optimization seems overly complicated and not well justified. There are likely better system-level solutions that would perform at least as well as genetic algorithms.

- It would be great if the paper could include a thorough evaluation of the points made in Figures 1-3, rather than just doing so for one or two models, because those points are key to the contributions of the paper. Some of the models used for evaluation might be outdated. It is best to include recent models such as BERT.

Comments for author
-------------------
The key insight of Pollux is that the training process should adapt to changes of statistical efficiency. This leads to the design of a scheduler that is fundamentally superior to those that do not take statistical efficiency into account. I consider the definition of Goodput a major contribution of the paper. 

How well Pollux works depends on how common and significant the statistical accuracy changes during DNN training and how accurate one can estimate, predict, and maximize goodput. The paper motivates the work in Figure 1 and validates its models in Figures 2 and 3. But they are done on only one or two models. It would be great if a more thorough evaluations can be performed. For example, does the statistical accuracy change during BERT model training and does the model predict as accurately for BERT as it does for ResNet18? 

The formalization of the cluster-wide optimization uses weighted speedup on all jobs. Would it be better to look at the overall effectiveness; for example, the job completion time or the total amount of resources consumed to finish all training (to reach the desirable accuracy objectives)? It is hard in general to assign weights to jobs, especially if the amount of resources consumed fluctuates over time. 

Pollux uses a generic algorithm for global optimization. I wonder whether a simpler greedy algorithm would work equally well, if not better. For example, we can simply calculate the effectiveness of resource uses for each job and its project effectiveness of using additional resources. We can then prioritize on offering more resources to those jobs that can more effectively use them than those who are currently using the resources. This will lead to mostly local adjustment, which tends to introduce less overhead. In practice, there are also other constraints to consider, including locality and fairness, which makes the decision making process complicated.

A more interesting setting is cloud auto-scaling. The comparison to the baseline is not easy to interpret: Pollux can train ImageNet for 25 percent cheaper cost, with only a 6 percent longer completion time. Is this the best point in cost/completion time tradeoff? How much can Pollux save under the same completion time? Or how fast can Pollux finish training given the same cost?

Novelty
-------
3. New contribution

Experimental methodology
------------------------
3. Average

Writing quality
---------------
4. Well-written

Overall merit
-------------
3. Weak accept (OK paper, but I am not enthusiastic)

Reviewer expertise
------------------
2. Some familiarity



Review #228B
===========================================================================

Paper summary
-------------
This paper presents Pollux, a scheduler that co-optimizes cluster-wide
resource allocations among DL jobs and tunes learning rate and batch 
size for each job. Pollux defines goodput that takes into account both
system throughput and statistical efficiency as a performance metric 
for optimizing cluster scheduling. In particular, modeling statistical 
efficiency is based on the gradient noise scale, the amount of progress
made per training example with batch size m relative to initial batch
size m0, which is also used in AdaScale. Pollux reduces job completion 
time by 25-50% compared to Optimus and Tiresias in the testbed environment 
with 16 nodes, each of which has 4 GPUs. In addition, simulation 
experiments show the effects of workloads, job weights, and interference 
avoidance on scheduling, and the cost and performance tradeoff of 
cloud autoscaling.

Strengths
---------
 Consideration of statistical efficiency for scheduling jobs in a cluster

 Use of goodput that considers both statistical efficiency and system 
throughput as a metric to optimize

 Co-optimization of job-level and cluster-level scheduling

Significant Weaknesses
----------------------
- The key contribution regarding statistical efficiency 
comes from AdaScale. Pollux job scheduling heavily relies on AdaScale.

- The system depends on the fact that AdaScale works correctly.
How does one ensure that AdaScale works beyond the training jobs used in 
the experiments? 

- The system relies on starting with some initial learning rate and 
batch size. How does one find the initial learning rate and batch size? 

Typically, users run hyperparameter optimization jobs to find good
hyperparameters including the learning rate and batch size. Some jobs 
can be early terminated and selected jobs run to completion. 
It is not clear how Pollux works with these common scenarios.

Comments for author
-------------------
I really like that the work tackles the problem of scheduling
DL jobs in a cluster by modeling statistical efficiency. This problem
is challenging and has not been addressed by prior work. Unfortunately,
I cannot strongly argue for Pollux yet since it has non-negligible 
weaknesses to be addressed.

First, statistical efficiency is modeled based on the AdaScale work.
Since the statistical efficiency is the most interesting part, 
I feel like Pollux's contribution is to build a system around 
AdaScale. 

Second, this dependency also raises a question on the correctness of
the system. The system depends on the fact that AdaScale works
correctly. How does one ensure that the modeling works for 
other models that are not covered by experiments? 

Third, the system also assumes that it starts with reasonable initial 
learning rate and batch size. Pollux can grow batch size over time
but it cannot decrease batch size. In a cluster, typically users
run hyperparameter optimization jobs to find good batch size and 
learning rate, momentum, etc, and then run a training job to 
completion. It's not clear how Pollux interacts with hyperparameter
optimization jobs whose execution depends on a hyperparameter
optimization algorithm. 

There are magic parameters, GPUTIME_THRES, RESTART_PENALTY, 
LOW_UTIL_THRES, HIGH_UTIL_THRES, etc. 
The paper does not provide any guide on how to set these parameters.

* 3.2 Modeling System Throughput

- Modeling T_{grad} assumes linearity. But, when m becomes larger,
GPU becomes saturated, thus the assumption does not hold.


* 4 Pollux Design and Architecture

- It would be good to discuss how to extend Pollux to cover 
other hyperparameters in addition to the batch size and learning rate.


* 4.2 PolluxSched

- "decreasing the weight of jobs according to the amount of GPU-time
already spent on them" ->  This strategy does not sound good. The 
job will stay longer as it is in the later stage of training.

- "it may be more cost-effective to provision more cloud resources 
during the later iterations of a large training job" -> This
strategy and the above strategy are contradictory.


* 5 Evaluation

- Although there are testbed experiments, but the most part of 
the experiments are done on a simulator. It would be more interesting
to present experiment results with a real system rather than 
simulation results.

Novelty
-------
2. Incremental improvement

Experimental methodology
------------------------
3. Average

Writing quality
---------------
4. Well-written

Overall merit
-------------
2. Weak reject (This paper should be rejected, but I'll not fight strongly)

Reviewer expertise
------------------
4. Expert



Review #228C
===========================================================================

Paper summary
-------------
In shared DL clusters, state-of-the-art DL schedulers either rely on user to specify the number of GPUs needed, or can automatically adapt the resource (GPU) allocation for differentDL jobs to optimize a certain objective, e.g., average job completion time. This paper applies recent idea/insight from the ML literature that (1) there is delicate balance between the system throughput and the statistical efficiency, e.g., the larger the batch size, the higher the throughput, but the lower the statistical efficiency, both of which affect the training job competition time, (2) statistical efficiency tends to increase during training, making it efficient to use larger batch size in later training iterations.  It then proposes a new DL scheduler that automatically tunes the resource (GPU) allocation, batch size, and learning rates for DL jobs, which are generally difficult for the user to configure manually. 

Building on recent work for characterizing the statistical efficiency, the paper models both system throughput and efficiency as a function of batch size and allocated GPU resources, and develops (1) job-level optimization that determines the optimal batch size that maximizes the goodput of each DL job, and (2) cluster-wide optimization that maximizes the weighted job SPEEDUP relative to allocating 1 GPU per job, across all jobs., using a genetic algorithm that also takes into account configuration change penalty. 
  
Testbed and simulation results show the new DL scheduler significantly improves the average job completion time over prior art that do not adjust batch size by exploiting statistically efficiency.

Strengths
---------
 Improving DL cluster scheduling efficiency is an important problem. 

 The paper turns an interesting insight about DL training efficiency into a new DL cluster scheduler that outperforms prior art. 

 Evaluation via both testbed and simulation are well executed and the results are convincing.

Significant Weaknesses
----------------------
- The key insight was from [25, 3] which was ready published. 

- Evaluation did not show the new scheme which optimizes the goodput of jobs  achieves the same training accuracy despite its fast job completion time.

- Some detailed analysis of the results could be helpful. 

- The new scheduler assumes homogeneous GPU.

Comments for author
-------------------
I enjoyed reading the paper. Although the key insights about statistical efficiency of large-batch training were from earlier literature, I thought the paper did a fairly decent job turning the insight into a new working DL cluster scheduler that outperforms the prior art which were oblivious to statistical efficiency and batch resizing. 

One important evaluation metric that is missing is the model training accuracy. In particular, does incorporating statistical efficiency to optimize the goodput of jobs guarantee the training reaches the same model accuracy as before? The evaluation needs to show this, or do you have theoretical backings for this? 

One thing that is not so obvious from reading the paper is that how much of the final average job competition time improvement of Pollux over Optimus comes from higher throughput per iteration using larger batch size in later iterations of the training, and how much of it comes from the reduced number of iterations (from increased learning rate due to increased batch size). It would be helpful to analyze and understand the breakdown by seeing the decoupled contributions from the two factors.  

[25] did not list where it was published? 

How do you extend the Pollux to handle heterogeneous GPU clusters?

Novelty
-------
3. New contribution

Experimental methodology
------------------------
4. Good

Writing quality
---------------
3. Adequate

Overall merit
-------------
4. Accept (Good paper, I will advocate for it)

Reviewer expertise
------------------
3. Knowledgeable



Review #228D
===========================================================================

Paper summary
-------------
Pollux is a scheduling framework focused on clusters dedicated to deep learning jobs, which are resource intensive, long-running, and use expensive hardware accelerators. It consists of two components: an agent running with each job that continuously monitors the throughput and efficiency of that job and dynamically tunes the batch size and learning rate, and a scheduler that runs a genetic algorithm every so often to modify GPU allocations according to the current efficiency of each job (in other words, allocating more resources to jobs that can make use of them). Core pieces of the system are the use of previously-published "gradient noise scale" to measure efficiency for a given batch size, and the AdaScale optimizer to scale the learning rate according to gradient noise scale. Pollux uses these techniques to predict so-called goodput (throughput * efficiency) for a given batch size and GPU allocation, and thus dynamically find the best resource allocation for the job.

The evaluation compares with two other DL schedulers (Optimus and Tiresias) and uses a synthetic trace on a testbed of 64 GPUs as well as with a simulator. It shows that job completion time is lower with Pollux. Finally, the evaluation runs an ImageNet model in the cloud compared to [35] and shows it to be more cost-efficient.

Strengths
---------
The paper is well-written and improving resource efficiency and job completion times for DL jobs seems a good problem to tackle. The evaluation has been performed carefully and I think the write-up might be mostly sufficient for reproducibility of the experiments, which is commendable. I am not qualified to judge the novelty of the ideas, but the paper makes a good case for taking an original approach to the problem.

Significant Weaknesses
----------------------
Although the work is positioned as a cluster scheduling framework, it doesn't consider standard metrics of scheduler goodness, such as cluster-wide utilization, scheduling overhead and fairness. The genetic algorithm used to update resource allocations isn't motivated or examined in isolation.

Comments for author
-------------------
This paper does a nice job of being explicit about the various measures and derivations of settings and heuristics (there are 17 equations!) I like the transparency and precision of this approach (although it can be overwhelming for the reader). On the other hand, the paper is not nearly forthcoming enough about how the system actually works in the experimental evaluation, and for me that is a significant weakness.

For example, it would be good to report details of the resource profiles in the comparative experiments (similar to the graphs of Figure 10 for ImageNet training in the cloud). I note from Figure 10 that the number of nodes is only adjusted twice by Pollus in 4 hours of running time. If this is typical, then it begs the question of whether the cost of reporting metrics and running the allocation algorithm every minute is reasonable given the return. I would be interested to know detail of the batch sizes that Pollux selected and how resource allocations were changed throughout the lifetime of a job. Also, how many jobs were running simultaneously and what was the overall cluster resource utilization in these experiments?

The second main concern is that the paper doesn't look at any cluster-wide metrics, such as utilization or fairness. The overhead of the optimization algorithm is important to know, as well as how it scales with the size of the cluster and the number of jobs (I think this would be a very interesting experiment in fact).

Why did you pick a genetic algorithm to optimize global resource allocations, and what alternatives did you consider?

I was disappointed you only ran a single model in the cloud (which cloud, by the way, was this the 16 nodes on AWS?) The Or et al paper[35] runs CIFAR-10 in addition to ImageNet. They also report how long resources in the cluster go idle while the job transitions to a new resource allocation, which also seems a very relevant metric here.

In summary, it feels like this paper is primarily about the throughput prediction and dynamic adaptation of batch size and learning rate, with the approach of using this information in a cluster scheduler as a less well-baked application of the idea. As a non-expert on the ML side, I can't usefully assess the quality of that part of the work, but as a cluster scheduling contribution, although the idea seems promising, this paper falls somewhat short.

Novelty
-------
2. Incremental improvement

Experimental methodology
------------------------
4. Good

Writing quality
---------------
4. Well-written

Overall merit
-------------
2. Weak reject (This paper should be rejected, but I'll not fight strongly)

Reviewer expertise
------------------
1. No familiarity



Review #228E
===========================================================================

Paper summary
-------------
This paper introduces Pollux, which is a distributed cluster scheduler for deep learning training that optimizes the goodput of a set of training jobs. Unlike previous cluster schedulers in this space, which either conservatively treat the size of a job as fixed, or cavalierly change the size of a job without regard for the effect on convergence, Pollux builds on recent work (AdaScale [ICML 2020] and McCandlish et al.'s empirical model of large-batch training) that measure the statistical efficiency of training tunes the learning rate of a job in response to a change in batch size (e.g. by increasing the number of parallel processes). Pollux builds a simple piecewise linear model of job throughput (whose parameters are learned online), and combines it a measure of efficiency derived from AdaScale's notion of gain ratio ($r_t$) (or McCandlish et al.'s gradient noise scale), to predict the goodput of a job in a particular configuration. A simple search process identifies the optimal batch size to use to maximize goodput, and then Pollux uses AdaScale to set the learning rate. Given a set of jobs and candidate resource assignments, a genetic algorithm attempts to optimize the average expected parallel speedup of those jobs in terms of their goodput. The genetic algorithm also accounts for a simple job prioritization scheme (based on weights), and supports constraints that avoid coscheduling multiple large jobs on the same host that might interfere. Finally, Pollux can use its model to choose the appropriate number of GPUs to rent from a cloud provider in order to maximise expected utility: it typically rents additional nodes for a job as training progresses and the training process is able to benefit from larger batch sizes.

The evaluation uses a workload inspired by Microsoft deep learning cluster traces, where jobs (whose sizes and durations approximately match the Microsoft trace) are trained to convergence under Pollux, and compared with the results using Tiresias and Optimus. Pollux outperforms the other schedulers in terms of average and P99 job completion time, and makespan. Results are presented for a small cluster deployment, as well as larger scale simulation.

Strengths
---------
Pollux uses a principled approach to elastic scaling of deep learning jobs, which puts the usual concerns about effects on convergence to rest. The results genetic algorithm for cluster scheduling is a nice touch, and many of

Significant Weaknesses
----------------------
Relying on all jobs to use AdaScale as the optimization algorithm may limit the applicability of the proposed technique. While promising, it is neither yet clear whether it will be widely adopted, nor whether the next $k$ optimization algorithms to be invented will be compatible with Pollux's mechanisms.

Comments for author
-------------------
Thank you for submitting this paper to OSDI! I was pleased to finally see a paper that takes a principled approach to elastic scaling for deep learning jobs and Pollux appears to be a promising step in that direction. While I have some concerns, detailed below, I think this paper would be a strong addition to the program, and I am in favor of accepting it.

My main concerns are pragmatic: I am skeptical that many deep learning practitioners would, as of today, adopt a cluster scheduler that forces them to yield control of the optimization algorithm. AdaScale displays promising results in the ICML paper, but as far as I can tell it only compares to Momentum-SGD, and doesn't dominate (or at least isn't evaluated against) other commonly used optimization algorithms like Adam. Hopefully in a year or two if AdaScale becomes de rigeur then adopting Pollux will be much easier. Could you discuss how Pollux might be adopted gradually, sharing a cluster with jobs that are not "white boxes", and perhaps are statically provisioned? Alternatively, is it feasible that the benefits of Pollux would accrue if you only measured statistical efficiency but did not switch the optimization algorithm to AdaScale? Furthermore, having worked in multiple institutions where access to GPUs is the subject of some contention, it would be interesting if PolluxAgent could be implemented without trusting all users: in the current setup, users might be incentivized to spoof a job that reports perfect scaling and high reported statistical efficiency, in order to acquire more GPUs.

I appreciated the sensitivity analysis in the evaluation. Did you also investigate the sensitivity to (i) the scheduler frequency, and (ii) the restart penalty? I suspect that 30 seconds is very optimistic for checkpointing and restarting a process in a deep learning job on a new machine, and the cluster utilization might rely on being able to reschedule jobs every minute to achieve high utilization. On a related note, is it possible to predict the goodput trajectory (my understanding of AdaScale and gradient noise scale is that these provide instantaneous measures of efficiency, but the dynamics are less clear), or incorporate information about the underlying learning rate schedule to make better informed scheduling decisions?

Do you consider gradient aggregation as a complementary method to achieving larger batch sizes? The comment "If a job's batch size does not fit on a single GPU, we additionally enforce a minimum number of GPUs, such that the total batch size will fit on that many GPUs" in the setup for Optimus suggests that you do not. Gradient aggregation could be a cost-effective way to achieve larger batch sizes with fewer GPUs, and can work even if the micro-batch size is 1 on a single GPU, although it would require changes to your throughput model. I am slightly concerned that this penalizes Optimus in your evaluation, because it ought to have more flexibility to scale down certain jobs (although it's possible that Optimus overlooked this possibility too).

Finally, there is a lot of related work on applying genetic algorithms to various scheduling problems, although it has not been especially fashionable in recent years. Please cite some relevant papers in the Related Work section. It would be interesting if you could also include some results showing the sensitivity to the number of iterations of genetic algorithm: does it tend to converge in the time available, or would a lower scheduling frequency provide more opportunity to optimize?

Novelty
-------
3. New contribution

Experimental methodology
------------------------
4. Good

Writing quality
---------------
4. Well-written

Overall merit
-------------
4. Accept (Good paper, I will advocate for it)

Reviewer expertise
------------------
2. Some familiarity



Review #228F
===========================================================================

Paper summary
-------------
Pollux combines hyper-parameter tuning with cluster scheduling. The insight is that doing so is advantageous as Pollux, based on the load on the system, can collectively tune the batch-size, learning rate, and the resource available to improve the collective job completion times. 

To this effect, Pollux learns models to predict the throughput and statistical efficiency of a ML job for a given amount of resources, and uses a genetic algorithm to maximize goodput of the system.

Experiments on a testbed and on a simulator show the advantages of this approach.

Strengths
---------
An interesting take on the ML cluster scheduling problem with promising results.

Significant Weaknesses
----------------------
Experiments could evaluate the many design choices in more detail.

Comments for author
-------------------
Personally, I think that schedulers should not change the "semantics" of programs they schedule. So, the approach this paper takes is perhaps controversial - the batch size and learning rate schedules should be determined/tuned by data scientists than changed dynamically by the scheduler. But this choice is what makes this paper interesting! 

What one ultimately cares about in ML training is time to desired accuracy - this is determined by the number of inputs required to reach this accuracy (the statistical efficiency) and the speed with which the system can process these inputs (the system throughput). In ML training, these two are fundamentally tied as choices to increasing the system throughput, such as batch size, can decrease the statistical efficiency. Pollux relies on recent work to approximate net statistical efficiency with gradient-noise that can be measured per-step. This allows Pollux to model both statistical efficiency and throughput instantaneously and make the best resource allocation decisions. 

Figure 2b shows that the predicted statistical efficiency matches the actual gradient-noise. It would also be good to validate for the models that manipulating the gradient noise actually reduces the number of images/epochs required to achieve the desired accuracy. 

The throughput modeling in the paper requires more explanation. The $T_{sync}$ should account for both intra-node synchronization and intra-node synchronization. So, I was expecting the term to be $\alpha + \beta_{local} \Sigma_i a_i + \beta_{global} (A-1)$ where $A$ is the number of non-zero elements in $a$. 

Overall, it would be good if the paper evaluates these many design choices empirically. Why you do compare with Tiresias and Optimus, you should compare with different version of Pollux that make slightly different design decisions. This way, we can better understand what aspects of Pollux lead to the performance improvements over prior work.

Novelty
-------
3. New contribution

Experimental methodology
------------------------
3. Average

Writing quality
---------------
3. Adequate

Overall merit
-------------
3. Weak accept (OK paper, but I am not enthusiastic)

Reviewer expertise
------------------
2. Some familiarity



resp1 Response by Aurick Qiao <aurick.qiao@petuum.com>
---------------------------------------------------------------------------
Thank you for the excellent feedback. We will address it all in revising the paper, and try to answer concerns raised here.

**Pollux and AdaScale (Review-B&E):** We want to clarify the difference between Pollux's dependence on the Gradient Noise Scale, which is a general property of DL training, and Pollux's use of AdaScale for learning rate scaling. Pollux uses the Gradient Noise Scale, not AdaScale, to model statistical efficiency of DL training, which should work for DL training in general (confirmed for all workloads in Table-1). However, the learning rate should be re-scaled whenever Pollux changes the batch size, which we do using AdaScale. Current and future alternatives for learning rate scaling may be used instead, if they also perform well.

**Genetic algorithm (Review-A&D):** We chose a genetic algorithm due to the complex, discrete, and high-dimensional search space of cluster-wide resource allocations, with constraints such as interference avoidance (Sec-4.2.1). There may be heuristics-based approaches that also work, but we found it natural to apply genetic mutation/crossover operations in this scenario, and it converged to reasonable solutions within time limits.

## Review-A

Pollux considers system-level decisions by modeling system throughput (Sec-3.2) with respect to the number and placement of GPUs, in addition to batch size. Both the system and statistical aspects are critical components of our goodput model.

Although Figures 1-3 show data for only a few cases, we experimentally validated using all workloads described in Table-1, which covers a wide range.

We don't have data on how BERT's statistical efficiency changes over time. However, even if it doesn't, BERT can still benefit from Pollux by (1) automatically using a better batch size when its resource allocation changes due to changes in cluster load, and (2) receiving more resources while a competing job is in a low-efficiency stage of training.

## Review-B

For clarification, it is possible for Pollux to decrease the batch size when downsizing the number of GPUs due to increasing cluster load, with the initial batch size as a lower limit.

**Setting initial learning rate and batch size.** Larger batch sizes result in better parallelism, but smaller batch sizes are easier for users, since high accuracy can be achieved with less worry about learning rate scaling. Thus, we recommend using a small initial batch size, from reasonable guidelines in literature, and let Pollux handle scaling the batch size for better parallelism. The initial learning rate can also be drawn from literature, or by hyper-parameter tuning (see below).

**Relationship with hyper-parameter tuning.** As mentioned, we recommend a fixed initial batch size, while the hyper-parameter tuner searches for other hyper-parameters (including initial learning rate) by spawning each trial as a Pollux job. This approach can be used with bayesian tuners like TPE and SMAC. Multi-armed bandit approaches like HyperBand and ASHA may require early forecasts of each trial's final accuracy to early-stop unpromising trials. Compatibility between accuracy forecasting and Pollux's adaptive batch sizes merits further investigation.

**Linear model for $T_{grad}$.** We agree there are performance properties of GPUs not captured by our simple linear model. Still, we found it sufficient to yield performance improvements when optimized as part of goodput. One strength of our goodput model is its modularity, allowing the throughput portion to be replaced by hardware-specific models, without compromising the Pollux design.

**Decreasing job weights and increasing cloud resources.** These two mechanisms are aimed at different scenarios. Decreasing job weights prioritizes between small jobs and large jobs, offering a useful tuning knob for cluster operators that maintains cluster-wide performance (Sec-5.3.2). In the cloud scenario, we auto-scale a virtual cluster running one large job, so its weight has no effect. 

We will be happy to extend Sec-5.3.2 to cover additional Pollux parameters.

## Review-C

**Model training accuracy.** The JCT metric used in our evaluation is the wall-clock time to reach the validation metrics listed in Table-1.

**Sources of improvement.** From Sec-5.2.1, Pollux improves *throughput* by 1.2x and goodput by 1.4x over Optimus+Oracle, with the difference due to fewer epochs. We shall break-down the job completion-times in our paper.

## Review-D

**Scheduling frequencies.** For clarification, Figure-10 shows few resource reallocations because the cluster-size is determined by cloud auto-scaling (Sec-4.2.2). For shared-cluster workloads, we observe more frequent resource reallocations. Furthermore, models that take less time to train (like Cifar-10) may benefit from more frequent metrics reporting and resource reallocations.

**Cluster-wide metrics.** We believe avg-JCT, 99%tile-JCT, and makespan are relevant cluster-wide metrics following prior work on DL cluster scheduling. Indeed, one source of performance improvement is due to better resource utilization from dynamic scheduling. We agree that other metrics, such as fairness, are also desirable but are outside the scope of our paper.

## Review-E

**Gradient accumulation and Optimus.** Neither Optimus (from their performance model and source code at https://github.com/kzhang28/Optimus) nor Pollux account for gradient accumulation, although it may be incorporated into Pollux. In fact, we believe Optimus' design suggests its total batch size cannot be larger than the limit of a single GPU (jobs always start with a single GPU and the batch size is constant). In our evaluation, we removed this limitation for Optimus (with a minimum GPUs limit) to ensure a conservative comparison.

**Practicality of adoption.** Adaptive batch sizes can be disabled in our current implementation of Pollux to ease adoption. In this mode, the job is compatible with other optimizers that depend on a constant batch size. The resources of the job can still be dynamically optimized (together with other adaptive batch size jobs) by PolluxSched, which simply assumes goodput is equal to throughput for that job.

## Review-F

**Modeling synchronization time.** We found that increasing from 1-to-2 nodes had a disproportionately larger impact than increasing from 2-to-N nodes. Thus, we used $\alpha^{node}$ to model the impact of using 2 nodes, and $\beta^{node}$ to model the impact from using more than 2 nodes. 

We will be happy to extend Sec-5.3.2 to show how Pollux variants would perform.



Comment @A1 by Reviewer E
---------------------------------------------------------------------------
Thank you for your author response. The reviewers have read and considered it.


Comment @A2 by Reviewer E
---------------------------------------------------------------------------
Thank you again for the submission and your response to our reviews. While many of the reviewers found the elastic scaling aspects of the paper interesting, there was skepticism about how widely AdaScale would apply to the workloads in a production cluster, and whether the convergence properties of a different optimizer would be sufficient.

The cluster scheduler component provoked more concern, and we would encourage the authors to develop this section of the paper further in revising the paper. The reviewers did not feel that this part of the paper reached the expected standard for a cluster scheduling paper at OSDI, and lacked evaluation of the scheduler's properties (fairness, utilization, scheduling overhead, etc.) that are typical for other papers in this space.
\end{lstlisting}
